First- and Second-Order Bounds for Adversarial Linear Contextual Bandits

We consider the adversarial linear contextual bandit setting, which allows for the loss functions associated with each of $K$ arms to change over time without restriction. Assuming the $d$-dimensional contexts are drawn from a fixed known distribution, the worst-case expected regret over the course of $T$ rounds is known to scale as $\tilde O(\sqrt{Kd T})$. Under the additional assumption that the density of the contexts is log-concave, we obtain a second-order bound of order $\tilde O(K\sqrt{d V_T})$ in terms of the cumulative second moment of the learner's losses $V_T$, and a closely related first-order bound of order $\tilde O(K\sqrt{d L_T^*})$ in terms of the cumulative loss of the best policy $L_T^*$. Since $V_T$ or $L_T^*$ may be significantly smaller than $T$, these improve over the worst-case regret whenever the environment is relatively benign. Our results are obtained using a truncated version of the continuous exponential weights algorithm over the probability simplex, which we analyse by exploiting a novel connection to the linear bandit setting without contexts.

==> result_2.tex <==
 Algorithm without rejection that computes $\Sigma_t$ by MGR, contain $1/\lambda_{min}$ in the bound, with adaptive learning rate.
 
 
 
 \begin{algorithm}[H]
 	\caption{\clinexpr}
 	\label{alg:linexp3_gr}
 	\textbf{Parameters:}  $\eta>0$,  $\gamma>0$.\\
 	\textbf{Initialization:} Set $\htheta_{0,a} = 0$ for all $i\in[K]$.
 	\\
 	\textbf{For} $t = 1, \dots, T$:
 	\begin{enumerate}
 		\item Observe $X_t$,
 		\item  pick $Q_t$ from the distribution $p_t$, defined in (\ref{exp3}) over set $\Omega$,
 		\item draw $A_t$ from the policy defined as
 		\[
 		\pi_{t}\left(a\middle|X_t\right)= Q_{t,a},
 		\]
 		\item observe the loss $\loss_t(X_t,A_t)$ and compute $\htheta_{t,a}$ for all $a$,
 		\item Run Geometric resampling and compute $\hSp_{t}$.
 	\end{enumerate}
 \end{algorithm}




\vspace{.25cm}
\makebox[\textwidth][l]{
	\fbox{
		\begin{minipage}{.48\textwidth}
			\textbf{Matrix Geometric Resampling}
			\vspace{.1cm}
			\hrule
			\vspace{.1cm}
		%	\textbf{Input:} Density $p_t$.\\
			Draw $MN$ samples as $\{ \pa{X_{i}, Q_{i}}\}_{i = 1,\dots, MN}$. Let $c=\frac{1}{2}$.
			\textbf{For $m = 1, \dots, M$, do}:
			\begin{itemize}
				\item \textbf{For $n = 1, \dots, N$, do}:
			\begin{enumerate}
			%	\vspace{-2mm}
				\item Set $i = (m-1)N + n$
				\item Compute $Y_{n} = diag_a\pa{Q_{i,a}^2X_i X_i\transpose}$,
				\item Compute $Z_{n} = \prod_{j=1}^n \pa{1 - c Y_n }$,
			\end{enumerate}
			\item Set $\hSpm = c I + c \sum_{n=1}^N Z_n$.
			\end{itemize}
			\vspace{-2mm}
			\textbf{Return $\hSp = \frac{1}{m} \sum_{m=1}^M \hSpm$}.
		\end{minipage}
	}
}
\vspace{.25cm}
 
  \begin{theorem}\label{main_theorem_2}
 	Using  $\eta_t = \frac{1}{10}\pa{2dK\pa{\hL_{t-1}+1 + G_t}}^{-1/2}$, $M_t = \lceil \frac{24 \ln(dHT)}{\epsilon^2}\frac{4}{\lambda_t^2 \ln^2\frac{1}{\varepsilon \lambda_t}}\rceil $ and $N_t = \lceil \frac{2}{\lambda_t}\ln \frac{1}{\varepsilon \lambda_t} \rceil$, $\lambda_t = \pa{\hL_{t-1}+1}^{-1/2}$, $\varepsilon=1/T$ the regret bound of Algorithm~\ref{alg:linexp3_gr} can be bounded as $R_T = \widetilde{O}\sqrt{dK L^*_T}$.
 \end{theorem}
